Stress Testing Method for Scenario Based Testing of Automated Driving Systems

Classical approaches and procedures for testing of automated vehicles of SAE levels 1 and 2 were based on defined scenarios with specific maneuvers, depending on the function under test. For automated driving systems (ADS) of SAE level 3+, the scenario space is infinite and calling for virtual testing and verification. However, even in simulation, the generation of safety-relevant scenarios for ADS is expensive and time-consuming. This leads to a demand for stochastic and realistic traffic simulation. Therefore, microscopic traffic flow simulation models (TFSM) are becoming a crucial part of scenario-based testing of ADS. In this paper, a co-simulation between the multi-body simulation software IPG CarMaker and the microscopic traffic flow simulation software (TFSS) PTV Vissim is used. Although the TFSS could provide realistic and stochastic behavior of the traffic participants, safety-critical scenarios (SCS) occur rarely. In order to avoid this, a novel Stress Testing Method (STM) is introduced. With this method, traffic participants are manipulated via external driver DLL interface from PTV Vissim in the vicinity of the vehicle under test in order to provoke defined critical maneuvers derived from statistical accident data on highways in Austria. These external driver models imitate human driving errors, resulting in an increase of safety-critical scenarios. As a result, the presented STM method contributes to an increase of safety-relevant scenarios for verification, testing and assessment of ADS.

==> 03_Vissim.tex <==
\subsection{Traffic Flow Simulation with Vissim}

Vissim uses a microscopic, behavioural and time step-oriented simulation model. As part of the microscopic models, the drivers form together with the Vehicles the smallest unit that represent the flow of traffic and by appropriate Behaviour models can be controlled. The behaviour models are in vehicle follow-up models, Lane change models and route selection models are subdivided and thus form the core of the microscopic simulation \cite{trapp}. Microscopically means that each driver-vehicle unit (DVU) can be modelled individually and therefore each vehicle has a driving behaviour or a Combination of several driving behaviour parameters is assigned. DVU's can differ from each other distinguish and are moved during the simulation through the modelled road network. Behavioural means that certain behaviour patterns can be created for each individual driver \cite{vissim}. The individual DVU's have different properties, which is why they fall can be subdivided in following categories:

\begin{itemize}
	\item \textbf{Technical specification of a vehicle} 
	\begin{itemize}
		\item Vehicle length and weight
		\item Accelerating and decelerating ability
		\item Maximum velocity
		\item Current position of the vehicle in the network
		\item Curent speed and acceleration
	\end{itemize}
	\item \textbf{Behaviour of the DVU }
	\begin{itemize}
		\item Driver's ability to remember
		\item Driver psycho-physical perception thresholds
		\item Acceleration as a consequence of the desired speed and the current speed of the driver
	\end{itemize}
	\item \textbf{Interaction between the driver-vehicle units}
	\begin{itemize}
		\item Indicators for currently used network sections and next nodes
		\item Influences of the preceding and following vehicle
	\end{itemize}
\end{itemize}



==> 04_02_Software_Design.tex <==
\subsection{Software Framework for DSTM}

For the manipulation and control of traffic vehicles in surrounding area of the vehicle under test a software framework in C++ is developed. The goal of the framework is ...

 
In \ref{fig:softwareDesign} the framework design is presented as an class diagram. Upon initialization of the external dirver DLL in Vissim, DLLMain is executed and framework leverages that as an entry point for creating singleton instance of Injector class. It has responsibility of querying, holding and processing data. All Vissim calls to the DLL, both set and get functions, are displaced in Injector class so it possesses a full control over vehicle data flow. From Vissim perspective, Injector class encapsulates vehicle processing and acts as a black box module where the internal state of box is updated through the set function, and output of it is fetched through the get function. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%				Figure 1
% 
\input{figures/figure_3}
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The Injector class from \ref{fig:} is derived from InjectorAbstract class. This design choice is taken in order to provide a user with the simple playground and to avoid any unnecessary changes to the vehicle extraction. User has to implement Inject method which is pure virtual method of InjectorAbstract and all code relevant for the processing of a vehicle data is to be written here. User is provided with basic methods for accessing data structures of vehicles in either simple array or map where map placement resembles placement of vehicles relative to the ego vehicle on the road. 
All code placed in inject method is applied to the nearby vehicles of chosen ego vehicle. That is made possible through the control of whole data flow. We know when all relevant vehicles are extracted and the moment before their new data is requested by Vissim, code from Inject function is applied and changes are delivered back to the Vissim.
Framework user has only two methods to play with, and that is Injector constructor and inject method which he has to implement. Role of inject method is already discussed. In constructor user can specify different settings, for example, ego vehicle id, minimum threshold for surrounding vehicles, specify that only vehicles in front of ego are stored, number of steps after which changes are applied. These changes are specified by setting different flags for parent constructor.


==> 04_03_Test_Method.tex <==

\input{04_02_Test_Method_Description}

\input{04_03_Stress_Testing_Long_Direction}

\input{04_04_Acceleration_and_Deceleration_Behaviour}

\input{04_05_Stress_Testing_Lateral_Direction}

\input{04_06_Lane_Change_Behaviour}



==> 04_04_ScenarioDescription.tex <==
\section{Scenario Description and Testing}





\input{long_scenarios}

\input{lat_scenarios}



==> graphics/02_Stress_Testing_Method/subsection_StressTestingLong/relevant_STM_scenarios_old.pdf_tex.tex <==
%% Creator: Inkscape inkscape 0.92.3, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'relevant_STM_scenarios.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \newcommand*\fsize{\dimexpr\f@size pt\relax}%
  \newcommand*\lineheight[1]{\fontsize{\fsize}{#1\fsize}\selectfont}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{500.43846908bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.52993384)%
    \lineheight{1}%
    \setlength\tabcolsep{0pt}%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{graphics/02_Stress_Testing_Method/subsection_StressTestingLong/relevant_STM_scenarios.pdf}}%
    \put(0.3036323,0.2601454){\color[rgb]{0.16862745,0.16470588,0.16078431}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$T_{2,1}$\end{tabular}}}}%
    \put(0.31841229,0.20331754){\color[rgb]{0.16862745,0.16470588,0.16078431}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$T_{3,1}$\end{tabular}}}}%
    \put(0.54732833,0.31930156){\color[rgb]{0.16862745,0.16470588,0.16078431}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$T_{1,2}$\end{tabular}}}}%
    \put(0.5298213,0.26130956){\color[rgb]{0.16862745,0.16470588,0.16078431}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$T_{2,2}$\end{tabular}}}}%
    \put(0.51121997,0.20331754){\color[rgb]{0.16862745,0.16470588,0.16078431}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$T_{3,2}$\end{tabular}}}}%
    \put(0.72266338,0.31930156){\color[rgb]{0.16862745,0.16470588,0.16078431}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$T_{1,3}$\end{tabular}}}}%
    \put(0.74345281,0.26130956){\color[rgb]{0.16862745,0.16470588,0.16078431}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$T_{2,3}$\end{tabular}}}}%
    \put(0.73229682,0.20239655){\color[rgb]{0.16862745,0.16470588,0.16078431}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$T_{3,3}$\end{tabular}}}}%
    \put(0.01869801,0.25887249){\color[rgb]{0.16862745,0.16470588,0.16078431}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$EGO$\end{tabular}}}}%
    \put(0.16189155,0.37183314){\color[rgb]{0.16862745,0.16470588,0.16078431}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$d_{1}^{TVC}$\end{tabular}}}}%
    \put(0.2786709,0.39842714){\color[rgb]{0.16862745,0.16470588,0.16078431}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$d_{2}^{TVC}$\end{tabular}}}}%
    \put(0.33832726,0.42597347){\color[rgb]{0.16862745,0.16470588,0.16078431}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$d_{3}^{TVC}$\end{tabular}}}}%
    \put(0.34405828,0.3162771){\color[rgb]{0.16862745,0.16470588,0.16078431}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$d_{1,1}$\end{tabular}}}}%
    \put(0.34868516,0.51282633){\color[rgb]{0.16862745,0.16470588,0.16078431}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$dVC_{1}$\end{tabular}}}}%
    \put(0.48616737,0.45223402){\color[rgb]{0.16862745,0.16470588,0.16078431}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$d_{max}^{TVC}$\end{tabular}}}}%
    \put(0.88787273,0.3102886){\color[rgb]{0.16862745,0.16470588,0.16078431}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$Lane_{1}$\end{tabular}}}}%
    \put(0.88896681,0.25557895){\color[rgb]{0.16862745,0.16470588,0.16078431}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$Lane_{2}$\end{tabular}}}}%
    \put(0.88896681,0.20086974){\color[rgb]{0.16862745,0.16470588,0.16078431}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$Lane_{3}$\end{tabular}}}}%
    \put(0.55938963,0.51159308){\color[rgb]{0.16862745,0.16470588,0.16078431}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$d_{2}$\end{tabular}}}}%
    \put(0.76315541,0.51040113){\color[rgb]{0.16862745,0.16470588,0.16078431}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$d_{3}$\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=2]{graphics/02_Stress_Testing_Method/subsection_StressTestingLong/relevant_STM_scenarios.pdf}}%
    \put(0.18494004,0.14419035){\color[rgb]{0.16862745,0.16470588,0.16078431}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$d_{3,1}$\end{tabular}}}}%
    \put(0.20893518,0.12639652){\color[rgb]{0.16862745,0.16470588,0.16078431}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$dtc_{1,1}$\end{tabular}}}}%
    \put(0.27642102,0.10795977){\color[rgb]{0.16862745,0.16470588,0.16078431}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$dtc_{3,2}$\end{tabular}}}}%
    \put(0.3007153,0.08846316){\color[rgb]{0.16862745,0.16470588,0.16078431}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$dtc_{2,2}$\end{tabular}}}}%
    \put(0.32532235,0.07103401){\color[rgb]{0.16862745,0.16470588,0.16078431}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$d_{1,2}$\end{tabular}}}}%
    \put(0.40941812,0.05119652){\color[rgb]{0.16862745,0.16470588,0.16078431}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$d_{1,3}$\end{tabular}}}}%
    \put(0.43185776,0.03101421){\color[rgb]{0.16862745,0.16470588,0.16078431}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$d_{2,3}$\end{tabular}}}}%
    \put(0.45590819,0.0092234){\color[rgb]{0.16862745,0.16470588,0.16078431}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$d_{3,3}$\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=3]{graphics/02_Stress_Testing_Method/subsection_StressTestingLong/relevant_STM_scenarios.pdf}}%
    \put(0.16147388,0.16174537){\color[rgb]{0.16862745,0.16470588,0.16078431}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$d_{2,1}$\end{tabular}}}}%
  \end{picture}%
\endgroup%

